Benchmarking Large Multimodal Models against Common Corruptions

This technical report aims to fill a deficiency in the assessment of large multimodal models (LMMs) by specifically examining the self-consistency of their outputs when subjected to common corruptions. We investigate the cross-modal interactions between text, image, and speech, encompassing four essential generation tasks: text-to-image, image-to-text, text-to-speech, and speech-to-text. We create a comprehensive benchmark, named MMCBench, that covers more than 100 popular LMMs (totally over 150 model checkpoints). A thorough evaluation under common corruptions is critical for practical deployment and facilitates a better understanding of the reliability of cutting-edge LMMs. The benchmarking code is available at https://github.com/sail-sg/MMCBench

==> tables/speech2text_cross.tex <==
\begin{table*}[!t]
\centering
\caption{Performance comparison of various \textbf{speech-to-text} models evaluated by self-consistency scores (cross-modality) across different corruption intensities and data selection levels. Scores represent the average multiplied cosine similarities (max 1600) between the original speech and the transcriptions generated for the speeches under different corruption conditions.}
\vspace{0.1cm}
\label{tab:speech2text_cross}
\begin{threeparttable}
\begin{tabular*}{0.85\textwidth}{@{\extracolsep{\fill}}lcccccc}
\toprule
\multirow{2}{*}{Models} & \multicolumn{2}{c}{Hard} & \multicolumn{2}{c}{Random} & \multirow{2}{*}{Average} \\  \cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & Heavy & Light & Heavy & Light & \\
\midrule
\first Wav2vec2 Base~\cite{baevski2020wav2vec} & 88   & 18   & -9   & 121  & 54.50  \\
\second SeamlessM4T Medium~\cite{seamlessm4t2023} & 165  & 88   & -7   & -49  & 49.25  \\
\third Robust Wav2Vec2 Large~\cite{hsu2021robust}  & -29  & -1   & 52   & 165  & 46.75  \\
Conformer-Transducer XXLarge~\cite{gulati2020conformer} & 76   & 15   & 38   & 56   & 46.25  \\
Conformer-CTC Small~\cite{gulati2020conformer} & -19  & 52   & 60   & 89   & 45.50  \\
Whisper Tiny~\cite{radford2023robust} & 58   & 78   & -18  & 50   & 42.00  \\
Conformer-Transducer Large~\cite{gulati2020conformer} & -4   & -77  & 84   & 128  & 32.75  \\
Wav2Vec2 Conformer Rope Large~\cite{wang2020fairseq}   & -64  & 8    & 122  & 64   & 32.50  \\
Distil Medium~\cite{gandhi2023distilwhisper} & 1    & 43   & -10  & 69   & 25.75  \\
Hubert Large~\cite{hsu2021hubert} & 132  & -127 & 1    & 89   & 23.75  \\
Conformer-CTC XLarge~\cite{gulati2020conformer} & 22   & 10   & 78   & -15  & 23.75  \\
Conformer-CTC Large~\cite{gulati2020conformer} & -58  & 134  & -97  & 101  & 20.00  \\
Distil Large~\cite{gandhi2023distilwhisper} & 26   & -64  & 23   & 81   & 16.50  \\
Conformer-Transducer Medium~\cite{gulati2020conformer}      & -2   & 18   & 25   & 12   & 13.25  \\
Conformer-Transducer XLarge~\cite{gulati2020conformer}    & -13  & -83  & 4    & 138  & 11.50  \\
Whisper Small~\cite{radford2023robust} & -29  & 24   & 36   & 10   & 10.25  \\
FastConformer-CTC Large~\cite{rekesh2023fast} & -25  & -6   & 58   & -21  & 1.50   \\
Wav2Vec2 Large Self-Training~\cite{baevski2020wav2vec, xu2021self} & 23   & -42  & 8    & 17   & 1.50   \\
SpeechT5~\cite{ao2022speecht5} & -7   & -7   & 63   & -51  & -0.50  \\
Distil Small~\cite{gandhi2023distilwhisper} & 23   & -40  & -29  & 37   & -2.25  \\
Conformer-CTC Medium~\cite{gulati2020conformer} & 72   & 40   & -153 & 30   & -2.75  \\
Whisper Large~\cite{radford2023robust} & -30  & 21   & 10   & -15  & -3.50  \\
FastConformer-Transducer Large~\cite{rekesh2023fast}  & -32  & 5    & 7    & 5    & -3.75  \\
S2T Medium~\cite{wang2020fairseq} & 103  & 81   & 25   & -232 & -5.75  \\
Wav2Vec2 Large~\cite{baevski2020wav2vec} & 39   & -30  & 25   & -60  & -6.50  \\
FastConformer-Transducer XLarge~\cite{rekesh2023fast}  & 72   & -161 & -18  & 71   & -9.00  \\
S2T Small~\cite{wang2020fairseq} & -18  & 31   & 1    & -51  & -9.25  \\
Whisper Base~\cite{radford2023robust} & 7    & -48  & 60   & -58  & -9.75  \\
FastConformer-Transducer XXLarge~\cite{rekesh2023fast} & -48  & -12  & 28   & -33  & -16.25 \\
SeamlessM4T Large~\cite{seamlessm4t2023} & 18   & -153 & -29  & 92   & -18.00 \\
Whisper Medium~\cite{radford2023robust}                     & -8   & -48  & -51  & 28   & -19.75 \\
SeamlessM4T v2-Large~\cite{barrault2023seamless} & 111  & -74  & -74  & -53  & -22.50 \\
ESPnet~\cite{watanabe2018espnet, arora2023universlu, pmlr-v202-radford23a} & -10  & -72  & -42  & 4    & -30.00 \\
S2T Large~\cite{wang2020fairseq} & -146 & -114 & 65   & 65   & -32.50 \\
MMS 1B All~\cite{pratap2023mms} & -59  & -23  & -86  & -39  & -51.75 \\
FastConformer-CTC XLarge~\cite{rekesh2023fast}       & -125 & -70  & -12  & -9   & -54.00 \\
Wav2Vec2 Large XLSR~\cite{conneau2020unsupervised, grosman2021xlsr53-large-english} & -141 & 47   & -163 & -45  & -75.50 \\
Wav2Vec2 Conformer Rel Pos Large~\cite{wang2020fairseq}   & 74   & -119 & -162 & -124 & -82.75 \\
Conformer-Transducer Small~\cite{gulati2020conformer} & -80  & -161 & -11  & -80  & -83.00 \\
FastConformer-CTC XXLarge~\cite{rekesh2023fast} & -121 & -63  & -74  & -78  & -84.00\\
\bottomrule
\end{tabular*}
\begin{tablenotes}
\footnotesize
\item[1] The Conformer CTC/Transducers and FastConformer CTC/Transducers models here are sourced from NeMo~\cite{kuchaiev2019nemo}.
\end{tablenotes}
\end{threeparttable}
\end{table*}


==> tables/text2speech_cross.tex <==
\begin{table*}[!t]
\centering
\caption{Performance comparison of various \textbf{text-to-speech} models evaluated by self-consistency scores (cross-modality) across different corruption intensities and data selection levels. Scores represent the average multiplied cosine similarities (max 2300) between original transcriptions and the speeches generated for the transcriptions under different corruption conditions. The name in parentheses indicates the source from which the checkpoint for this model was obtained.}
\vspace{0.2cm}
\label{tab:text2speech_cross}
\begin{tabular*}{0.925\textwidth}{@{\extracolsep{\fill}}lcccccc}
\toprule
\multirow{2}{*}{Models} & \multicolumn{2}{c}{Hard} & \multicolumn{2}{c}{Random} & \multirow{2}{*}{Average} \\  \cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & Heavy & Light & Heavy & Light & \\
\midrule
\first SeamlessM4T Medium~\cite{seamlessm4t2023} & 71   & 46   & 129  & 197  & 110.75  \\
\second XTTS v2~\cite{xtts}      & 98   & 95   & 40   & 78   & 77.75   \\
\third SeamlessM4T Large~\cite{seamlessm4t2023}        & 23   & 44   & -3   & 149  & 53.25   \\
FastSpeech2 (Facebook)~\cite{ren2020fastspeech, wang2020fairseq}     & 19   & 45   & 7    & 137  & 52.00   \\
SpeechT5~\cite{ao2022speecht5}              & -112 & 233  & 129  & -95  & 38.75   \\
SeamlessM4T v2 Large~\cite{barrault2023seamless}      & -86  & 87   & -15  & 154  & 35.00   \\
MMS~\cite{pratap2023mms}              & 154  & 4    & -75  & 19   & 25.50   \\
Tacotron2 (SpeechBrain)~\cite{shen2018natural, speechbrain}     & -35  & -105 & 79   & 140  & 19.75   \\
Fastpitch (NeMo)~\cite{lancucki2021fastpitch, kuchaiev2019nemo}       & -112 & 143  & 16   & -30  & 4.25    \\
VITS (NeMo)~\cite{kim2021conditional, kuchaiev2019nemo}           & 6    & -179 & 55   & 36   & -20.50  \\
MixerTTS-X (NeMo)\cite{tatanov2022mixer, kuchaiev2019nemo}     & -48  & -113 & -96  & 60   & -49.25  \\
Tacotron2 (NeMo)~\cite{shen2018natural, kuchaiev2019nemo}          & 72   & -75  & -27  & -189 & -54.75  \\
MixerTTS (NeMo)~\cite{tatanov2022mixer, kuchaiev2019nemo}      & -67  & -88  & -101 & -45  & -75.25  \\
ESPnet2~\cite{watanabe2018espnet}  & -123 & -82  & 78   & -313 & -110.00 \\
\bottomrule
\end{tabular*}
\end{table*}

